Coend calculus

The book formerly known as "This is the (co)end, my only (co)friend".

==> chapters/PP-leitfaden.tex <==
\cleardoublepage
\thispagestyle{empty}
\vspace*{\fill}

\begin{figure}[h]
	\begin{center}
		\begin{tikzpicture} [
				node distance=.75in and .5in,
				chapter number/.style={
						anchor=south,
						fill=gray!70,
						font=\color{white}\bfseries\scriptstyle,
						inner sep=0,
						outer sep=0,
						minimum size=.15in,
					},
				chapter name/.style={
						align=center,
						draw=gray!70,
						thick,
						rectangle,
						rounded corners,
						fill=gray!10,
						inner sep=.125in,
					},
			]

			\begin{scope}[every node/.style=chapter name]
				\node (1) {Dinaturality\\and coends};
				\coordinate [below=of 1] (porch);
				\begin{scope} [node distance=.166in]
					\node [left=2cm of porch] (2) {Yoneda\\and Kan};
					\node [right=4cm of 2] (A) {Category theory\\fundamentals};
				\end{scope}
				\node [below=of porch] (3) {Nerves\\and realisations};
				\coordinate [below=of 3] (basement);
				\begin{scope} [node distance=.125in]
					\node [left=of 3] (5) {Profunctors};
					\node [right=1cm of 3] (4) {Weighted\\co\fshyp{}limits};
				\end{scope}
				\coordinate [below=of basement] (garage);
				\begin{scope} [node distance=.75in]
					\node [below=4cm of 5] (6) {Operads};
					\node [below=2cm of 3] (8) {Addenda};
					\node [below=4cm of 4] (7) {Higher co\fshyp{}ends};
				\end{scope}
			\end{scope}

			\begin{scope}[
					every path/.style={
							draw=gray!10!black,
							->,
							>=stealth',
							thick,
						},
				]
				\path (1) -- (2);
				\path (2) -- (3);
				\path (3) -- (4);
				\path (4) -- (7);
				\path (2) -- (5);
				\path (5) -- (6);
				\path (5) -- (8);
				\path (4) -- (8);
				\begin{scope}[
						every path/.append style={
								dashed,
							},
					]
					\path (A) -- (1);
					\path (A) -- (2);
					\path (A) -- (3);
					\path (A) -- (4);
				\end{scope}
			\end{scope}

			\begin{scope}[every node/.style=chapter number]
				\node at (1.45)  {\oldstylenums{1}};
				\node at (2.135) {\oldstylenums{2}};
				\node at (3.90)  {\oldstylenums{3}};
				\node [below] at (4.-45) {\oldstylenums{4}};
				\node [below] at (5.-135) {\oldstylenums{5}};
				\node at (6.45)  {\oldstylenums{6}};
				\node at (7.25)  {\oldstylenums{7}};
				\node at (A.45)  {A};
				\node [below] at (8.-45)  {\oldstylenums{8}};
			\end{scope}

		\end{tikzpicture}
	\end{center}
	\caption*{Conceptual dependencies between the chapters.}
\end{figure}
\vspace*{\fill}
\cleardoublepage

